ACT: Empowering Decision Transformer with Dynamic Programming via Advantage Conditioning

Decision Transformer (DT), which employs expressive sequence modeling techniques to perform action generation, has emerged as a promising approach to offline policy optimization. However, DT generates actions conditioned on a desired future return, which is known to bear some weaknesses such as the susceptibility to environmental stochasticity. To overcome DT's weaknesses, we propose to empower DT with dynamic programming. Our method comprises three steps. First, we employ in-sample value iteration to obtain approximated value functions, which involves dynamic programming over the MDP structure. Second, we evaluate action quality in context with estimated advantages. We introduce two types of advantage estimators, IAE and GAE, which are suitable for different tasks. Third, we train an Advantage-Conditioned Transformer (ACT) to generate actions conditioned on the estimated advantages. Finally, during testing, ACT generates actions conditioned on a desired advantage. Our evaluation results validate that, by leveraging the power of dynamic programming, ACT demonstrates effective trajectory stitching and robust action generation in spite of the environmental stochasticity, outperforming baseline methods across various benchmarks. Additionally, we conduct an in-depth analysis of ACT's various design choices through ablation studies. Our code is available at https://github.com/LAMDA-RL/ACT.

==> tables/delayed_perf.tex <==
\begin{table}[htbp]
    \caption{Normalized score on delayed reward tasks, where \textit{hc}, \textit{hp}, and \textit{wk} stand for halfcheetah, hopper, and walker2d. \textit{Med} and \textit{exp} are abbreviations for medium and expert. The average and std are taken across 4 independent runs.}
    \label{tab:delayed_perf}
    \centering
    \scalebox{0.9}{
    \begin{small}
    \begin{tabular}{c|llll}
    \toprule[1.0pt]
        Dataset & CQL & IQL & DT & ACT\\
        \midrule
        hp-med & $ 46.1_{\pm2.9} $ & $ 32.4_{\pm7.7} $ & $ \bm{65.7_{\pm1.4}} $ & $ 49.4_{\pm1.5} $\\
        hp-med-exp & $ 0.8_{\pm0.3} $ & $ 97.6_{\pm14.8} $ & $ \bm{106.6_{\pm3.7}} $ & $ 95.4_{\pm13.9} $\\
        wk-med & $ -0.3_{\pm0.1} $ & $ 53.2_{\pm6.7} $ & $ 72.1_{\pm4.3} $ & $ \bm{73.8_{\pm1.9}} $\\
        wk-med-exp & $ 7.0_{\pm6.4} $ & $ 67.4_{\pm22.1} $ & $ 107.4_{\pm0.3} $ & $ \bm{108.1_{\pm0.2}} $\\
        \midrule
        Average & $13.4$&$62.7$&$\bm{88.0}$& $81.7$\\
        \bottomrule[1.0pt]
    \end{tabular}
    \end{small}
    }
\end{table}

==> tables/deterministic_mujoco_perf.tex <==
\begin{table*}[htbp]
\caption{Normalized score on deterministic Gym MuJoCo tasks, with datasets from D4RL. The performances of QDT and EDT are taken from their original paper, and the numbers for other baselines are taken from ~\cite{xql}. For ACT and DT, we use our own implementations and report the average performance and the standard deviation of the final checkpoint across 10 evaluation episodes and 5 seeds. We bold the highest score among sequence-modeling methods, and add background shading to the highest score among all methods.}
\label{tab:deterministic_gym_perf}
\centering
\begin{small}
\scalebox{0.9}{
\begin{tabular}{ccrrrrr|rrrr}
\toprule[1.5pt]
\multicolumn{2}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{5}{c}{Markovian}& \multicolumn{4}{c}{Non-Markovian} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-11}

& &\multicolumn{1}{r}{CQL}   & \multicolumn{1}{r}{Onestep RL} & \multicolumn{1}{r}{IQL} &\multicolumn{1}{c}{10\% BC} & \multicolumn{1}{r}{RvS} &\multicolumn{1}{r}{DT}&\multicolumn{1}{r}{QDT}&\multicolumn{1}{r}{EDT}&  \multicolumn{1}{r}{ACT}\\ 
\midrule

\multicolumn{1}{c}{halfcheetah} & \multicolumn{1}{c}{\multirow{3}{*}{medium}} &$44.0$\,\,& $48.4$\,\,   &$47.4$  &$42.5$  &$41.6$  & $42.6$   &$42.4\pm\,\,\, 0.5$ &$42.5\pm\,\, 0.9$& \colorbox{gray!30}{$\bm{49.1\pm\, 0.2}$} \\

\multicolumn{1}{c}{hopper} &&$58.5$\,\, &$59.6$\,\,  & $66.2$   &$56.9$  &$60.2$  & $62.3$   &$60.7\pm\,\,\, 5.0$ &$63.5\pm\,\, 5.8$& \colorbox{gray!30}{$\bm{67.8\pm\, 5.5}$} \\

\multicolumn{1}{c}{walker2d} &&$72.5$\,\, & \colorbox{gray!30}{$81.8$}   &$78.3$  & $75.0$   &$71.7$  &$74.3$  &$63.7\pm\,\,\, 6.4$ &$72.8\pm\,\, 6.2$& $\bm{80.9\pm\, 0.4}$\,\,\\
\midrule

\multicolumn{1}{c}{halfcheetah} & \multicolumn{1}{c}{\multirow{3}{*}{medium-replay}} & \colorbox{gray!30}{$45.5$} &$38.1$\,\,  &$44.2$  & $40.6$   &$38.0$  &$36.9$  &$32.8\pm\,\,\, 7.3$ &$37.8\pm\,\, 1.5$& $\bm{43.0\pm\, 0.4}$\,\,\\

\multicolumn{1}{c}{hopper} &&$60.9$\,\, & $97.5$\,\,   &$94.7$  &$75.9$  &$73.5$  & $75.8$   &$38.7\pm26.7$ &$89.0\pm\,\, 8.3$& \colorbox{gray!30}{$\bm{98.4\pm\, 2.4}$} \\

\multicolumn{1}{c}{walker2d} && \colorbox{gray!30}{$77.2$} &$49.5$\,\, &$73.8$  &$62.5$  &$60.6$  & $59.4$   &$29.6\pm15.5$ & $\bm{74.8\pm4.9}$ &$56.1\pm10.9$\,\,  \\
\midrule

\multicolumn{1}{c}{halfcheetah} & \multicolumn{1}{c}{\multirow{3}{*}{medium-expert}} &$91.6$\,\,& $93.4$\,\,   &$86.7$  & $92.9$   &$92.2$  &$86.3$  &$-$ &$-$ &\colorbox{gray!30}{$\bm{96.1\pm\, 1.4}$}\\

\multicolumn{1}{c}{hopper} && $105.4$\,\, &$103.3$\,\, &$91.5$ & $110.9$  &$101.7$ &$104.2$ &$-$ &$-$& \colorbox{gray!30}{$\bm{111.5\pm\, 1.6}$} \\

\multicolumn{1}{c}{walker2d} &&$108.8$\,\,& $113.0$\,\,  &$109.6$ & $109.0$  &$106.0$ &$107.7$ &$-$ & $-$&\colorbox{gray!30}{$\bm{113.3\pm \, 0.4}$}\\

\bottomrule[1.5pt]
\end{tabular}
}
\end{small}
\end{table*}


==> tables/hyper-parameters_act.tex <==
\begin{table}[htbp]
\caption{Hyper-parameters of ACT}
\label{apptab:hyper-parameters_act}
\centering
\begin{normalsize}
\begin{tabular}{c|c|c}
\toprule[1.5pt]
\textbf{Architecture} &\textbf{Hyper-parameters} & \textbf{Value}\\
\midrule
\multirow{6}{*}{$Q_\theta$ and $V_\psi$} & \# of hidden layers & 3\\
&Layer width & 256\\
&Learning rate &$3\times 10^{-4}$\\
&Discount $\gamma$ & 0.99\\
&Polyak coeff. & 0.005\\
&Batch size & 256\\
&Training steps & 200k\\
&Expectile $\sigma_1$ & 0.5 or 0.7\\
\midrule
\multirow{5}{*}{$c_\phi$} & \# of hidden layers & 3\\
& Layer width & 256\\
&Learning rate & $3\times 10^{-4}$\\
&Batch size & $256$\\
&Training steps & 500k\\
&Expectile $\sigma_2$ & 0.98\\
&Weight decay & $5\times 10^{-4}$\\
\midrule
\multirow{14}{*}{ACT}&\# of encoder layers & 3\\
&\# of decoder layers & 3\\
&\# of attention heads & 1\\
&Embedding dimension & 128 \\
&Nonlinearity function & ReLU \\
&Batch size & 64\\
&Context length & 20 \\
&Dropout & 0.1 \\
&Learning rate & $10^{-4}$\\
&Lr Warmup steps & 10000\\
&Grad norm clip & 0.25 \\
&Weight decay & $10^{-4}$ \\
&Adam betas & [0.9, 0.999]\\
&Training steps & 500k or 1M\\
\bottomrule[1.5pt]
\end{tabular}
\end{normalsize}
\end{table}

==> text/0.abstract.tex <==
Decision Transformer~(DT), which employs expressive sequence modeling techniques to perform action generation, has emerged as a promising approach to offline policy optimization. However, DT generates actions conditioned on a desired future return, which is known to bear some weaknesses such as the susceptibility to environmental stochasticity. To overcome DT's weaknesses, we propose to empower DT with dynamic programming. Our method comprises three steps. First, we employ in-sample value iteration to obtain approximated value functions, which involves dynamic programming over the MDP structure. Second, we evaluate action quality in context with estimated advantages. We introduce two types of advantage estimators, IAE and GAE, which are suitable for different tasks. Third, we train an Advantage-Conditioned Transformer~(ACT) to generate actions conditioned on the estimated advantages. Finally, during testing, ACT generates actions conditioned on a desired advantage. Our evaluation results validate that, by leveraging the power of dynamic programming, ACT demonstrates effective trajectory stitching and robust action generation in spite of the environmental stochasticity, outperforming baseline methods across various benchmarks. Additionally, we conduct an in-depth analysis of ACT's various design choices through ablation studies.

% demonstrates robust action generation in spite of environmental stochasticity and effective trajectory stitching\zzz{any evidence?} which boosts performance.


% Decision Transformer~(DT), which employs expressive sequence modeling techniques to perform action generation by conditioning on the desired returns, has emerged as a promising approach to offline policy optimization. 
% However, it is known to bear weaknesses, particularly the susceptibility to environmental stochasticity.
% To overcome its weaknesses, we propose Advantage-Conditioned Transformer~(ACT), a method that empowers DT with dynamic programming by conditioning on the advantages of taking specific actions given the context.
% To achieve this, we first employ in-sample value iteration to obtain the estimations of both the state-action value function $\hat{Q}$ and the state value function $\hat{V}$, which involves dynamic programming over the MDPs structure.
% Next, we label the transitions in the offline dataset with their estimated advantages.
% One method of which is to compute the advantage as the difference between $\hat{Q}$ and $\hat{V}$, but we further extend the calculation to Generalized Advantage Estimation~(GAE) to provide a more versatile estimation of the advantage which is suitable for a wider range of tasks such as the delayed reward tasks.
% By leveraging the power of dynamic programming, ACT demonstrates robust action generation in spite of environmental stochasticity and effective trajectory stitching which contributes to the success of offline reinforcement learning.
% Through extensive experiments, we find that ACT outperforms the baseline methods in deterministic and stochastic benchmarks, justifying the incorporation of dynamic programming.
% Additionally, we conduct an in-depth analysis of ACT's various design choices through ablation study. 

==> text/1.introduction.tex <==
Reinforcement Learning~(RL) optimizes policies by interacting with the environment often for millions of steps~\cite{sac}. Such enormous sample complexity prohibits RL from real-world applications such as robotics and healthcare. As an alternative, offline RL optimizes policies with a pre-collected dataset~\cite{levine_survey} and has gained increasing attention in recent years for its potential in real-life scenarios~\cite{robotics1,healthcare1}.
% real-world applications such as robotics~\cite{robotics1,robotics2,robotics3} and healthcare~\cite{healthcare1,healthcare2}.

Building upon online RL, a substantial amount of algorithms addresses offline policy optimization following the spirit of dynamic programming~\cite{levine_survey}, i.e. leveraging the structure of Markov Decision Process~(MDP) and employing Bellman update to derive value estimates for subsequent policy optimization~\cite{bcq,iql,onestep_rl}.

In the meantime, the past few years have witnessed huge success in applying sequence modeling to natural language processing~\cite{attention_is_all_you_need, gpt3}.
In light of the similarity between language sequences and RL trajectories, a lot of works have explored the idea of modeling RL trajectories using sequence modeling approaches.
For example, Decision Transformer~(DT)~\cite{dt} models offline trajectories extended with the sum of the future rewards along the trajectory, namely the return-to-go~(RTG). 
RTG characterizes the quality of the subsequent trajectory, and DT learns to predict future actions given RTG. During testing, we deliberately provide DT with a high RTG to generate an above-average action.
This approach, known as \textit{conditional sequence generation}, has achieved remarkable success in offline policy optimization.

However, we note that RTG-conditioned generation is defective.
Firstly, RTG is a hindsight indicator of a complete trajectory. It cannot be computed if we only have incomplete trajectory segments. Besides, we cannot ascertain the most suitable target RTG during testing, which poses a risk of choosing an inappropriate one and degenerating the performance. Secondly, conditioning on RTG fails to leverage the inherent structure of MDPs and cannot stitch trajectory as classical offline RL methods do. Therefore, DT cannot achieve much better performance than RL methods.
Lastly, when the environment is stochastic, DT tends to exploit the occasional high return in the offline dataset mistakenly, which negatively impacts its performance. 
% This phenomenon is also known as the optimism bias~\cite{optimism_bias} for sequence modeling methods.

In this paper, we present Advantage-Conditioned Transformer~(ACT), a method that empowers the traditional DT with dynamic programming to effectively address the above-mentioned challenges. To tackle the limitations of conditioning on RTG, we introduce advantages as replacements.
To obtain the advantage, we first approximate value functions with separate neural networks.
Afterward, we introduce two types of advantage estimation, namely IAE and GAE, which exhibit different characteristics and prove to be suited for different types of tasks.
We evaluate ACT in various benchmarks including those with stochastic dynamics and delayed rewards.
The results show that, with suitable advantage estimation, ACT significantly outperforms existing sequence modeling techniques and achieves performance on par with state-of-the-art offline RL methods.
We also carried out extensive ablation studies to highlight the effectiveness of the design choices of ACT.
Overall, our empirical results affirm the efficacy of the proposed method in addressing the limitations of DT and showcase its potential in applications.


==> text/2.preliminaries.tex <==
\subsection{Offline Reinforcement Learning}
A Markov Decision Process~(MDP) can be denoted by a six-tuple $\langle \mathcal{S}, \mathcal{A}, T, \mathcal{R}, \rho_0, \gamma \rangle$, where $\mathcal{S}$ stands for the state space, $\mathcal{A}$ is the action space, $T$ is the transition function, $\mathcal{R}$ is the reward function, $\rho_0$ is the initial distribution of states, and $\gamma\in[0, 1)$ denotes the discount factor of future rewards. For states $s,s'\in\mathcal{S}$ and $a\in\mathcal{A}$, $T(s'|s, a)$ specifies the transition probability of arriving at state $s'$ after taking action $a$ at state $s$, and $\mathcal{R}(s, a)$ gives the immediate reward of taking action $a$ at state $s$. A policy $\pi$ is a function mapping states to action distributions, and $\pi(a | s)$ is the probability to take action $a$ at state $s$.
The policy's quality is measured by the expected discounted return $J(\pi)=\mathbb{E}_\pi\left[\sum_{t=0}^\infty\gamma^{t}r_t\right]$, where $r_t=\mathcal{R}(s_t,a_t)$ is the reward obtained at time $t$, $s_t, a_t$ are the state and action at time $t$, respectively, and the expectation is taken w.r.t. the stochastic interaction of the policy $\pi$ and the MDP environment.
In offline RL, an agent is expected to learn a policy maximizing the expected discounted return with a static dataset $\mathcal{D}$. Typically, $\mathcal{D} = \{\tau_k\}_{k=1}^{K}$ is composed of $K$ trajectories $\tau_k$ collected by a behavior policy $\beta$, where $\tau_k=\{s^k_t, a^k_t, r^k_t\}_{t=0}^{N_k-1}$, $s^k_t$, $a^k_t$, and $r^k_t$ denote state, action, and reward at timestep $t$ of the $k$-th trajectory, respectively, and $N_k$ is the trajectory length of the $k$-th trajectory.

% Offline RL can be seen as an extreme case of off-policy RL~\cite{bcq} with additional challenges such as the absence of online corrective feedback for overestimated value functions.

\subsection{Dynamic Programming in RL}\label{sec2.2}
A commonly used categorization of deep RL algorithms is by their optimization paradigm, either \textit{policy gradient} or \textit{approximate dynamic programming}~\cite{levine_survey}. The former derives the gradient of RL objectives w.r.t. the policy via the policy gradient theorem~\cite{policy_gradient} and improves the policy via gradient ascent. The latter derives the optimal policy exploiting the value function. The value functions of a policy $\pi$ are defined recursively:
$$
    \begin{aligned}V^\pi(s)&=\mathbb{E}_{a\sim\pi(\cdot|s)}\left[Q^\pi(s,a)\right],\\
    Q^\pi(s, a)&=\mathcal{R}(s,a)+\gamma\mathbb{E}_{s'\sim T(\cdot|s,a)}\left[V^\pi(s')\right].
    \end{aligned}
$$
Solving the value function with dynamic programming, we can derive an improved policy by increasing the probability of selecting actions with positive advantages, where the advantage of an action $a$ at state $s$ is $A^{\pi}(s,a)=Q^{\pi}(s,a)-V^{\pi}(s)$. We can get the optimal policy by repeating this process, which is called policy iteration. Alternatively, we can use the value iteration and directly solve the optimal value functions $V^*$ and $Q^*$ with dynamic programming, where
$$
    \begin{aligned}
    V^*(s)&=\max_a Q^*(s,a),\\
    Q^*(s, a)&=\mathcal{R}(s,a)+\gamma\mathbb{E}_{s'\sim T(\cdot|s,a)}\left[V^*(s')\right].
    \end{aligned}
$$
The optimal policy $\pi^*$ is then obtained by greedily selecting the action $a$ with optimal value $Q^*(s,a)$ at all state $s\in\mathcal{S}$. 
% The optimal policy is then obtained as $\pi^*(a|s)=\mathbb{I}(a=\arg\max_{a'}Q^*(s,a'))$\zzz{The formula is wrong when there exist multiple optimal actions}, where $\mathbb{I}$ is the indicator function that takes value $1$ if the condition holds and $0$ otherwise.
% \begin{equation}
%     \begin{aligned}
%     V^\pi(s_t)&=\mathbb{E}_{\tau\sim p_\pi(\cdot|s_t)}\left[\sum_{t'=t}^H\gamma^{t'-t}r_{t'}\right]\\
%     Q^\pi(s_t, a_t)&=\mathbb{E}_{\tau\sim p_\pi(\cdot|s_t, a_t)}\left[\sum_{t'=t}^H\gamma^{t'-t}r_{t'}\right],\\
%     \end{aligned}
% \end{equation}
% where $p_\pi(\cdot|s_t)$ and $p_\pi(\cdot|s_t, a_t)$ denote the distribution of trajectories that starts from $s_t$ and $(s_t, a_t)$, respectively. There exists a recursive structure in Q-value functions:
% \begin{equation}\label{eq:bellman_exp}
%     \begin{aligned}
%     Q^\pi(s_t, a_t) &= r_t+\\
%     &\gamma\mathbb{E}_{s_{t+1}\sim T(\cdot|s_t, a_t), a_{t+1}\sim \pi(\cdot|s_{t+1})}[Q^\pi(s_{t+1}, a_{t+1})].
%     \end{aligned}
% \end{equation}
% We can use the \text{Bellman operator} $\mathcal{B}^\pi$ to express this structure: $Q^\pi=\mathcal{B}^\pi Q^\pi$. 
% In RL, policy iteration works by iteratively applying Equation~\eqref{eq:bellman_exp} to obtain Q-value estimation $\hat{Q}^\pi$ for the current policy $\pi$, and afterward use the estimation to update the policy $\pi_{\text{new}}(a|s) = \delta(a=\arg\max_{a'} \hat{Q}^\pi(s, a))$. 
% Another DP-based algorithm is value iteration, which can be used to directly estimate the optimal value function:
% \begin{equation}
%     \begin{aligned}
%     Q^\star(s_t, a_t) &= r_t + \\
%     &\gamma \mathbb{E}_{s_{t+1}\sim T(\cdot|s_t, a_t)}\left[\max_{a_{t+1}\in\mathcal{A}}Q^\star(s_{t+1}, a_{t+1})\right].\\
%     \end{aligned}
% \end{equation}
% which can be expressed as $Q^\star=\mathcal{B}^\star Q^\star$.

Compared with policy gradient methods, dynamic programming leverages the structure of MDP, gaining advantages in efficiency and performance empirically. 

\subsection{Decision Transformer}
% In recent years, practitioners have successfully extended the application of high-capacity sequence modeling architectures to control tasks. 
One of the pioneering works of solving control tasks with high-capacity sequence modeling networks is the Decision Transformer~(DT)~\cite{dt}. For each trajectory $\tau\in\mathcal{D}$, DT first computes the RTG $\hat{R}_t$ for each timestep $t$ by summing up the rewards along the future trajectory, $\hat{R}_t=\sum_{t'=t}^{N-1}r_{t'}$, where $N$ is the trajectory length. Later, DT fits a GPT-2 model~\cite{gpt2} on the offline trajectories augmented with RTGs, $\tau^{\mathrm{RTG}} = \{\hat{R}_t, s_t, a_t\}_{t=0}^{N-1}$.

During testing, DT first specifies the desired target return as $\hat{R}_0$, and executes the predicted action $\hat{a}_0$ given the history $(\hat{R}_0, s_0)$. After observing the new state $s_{1}$ and reward $r_0$, DT sets $\hat{R}_1=\hat{R}_0 - r_0$ and continues to predict the next action given the updated history $(\hat R_0,s_0,\hat R_1,s_1)$. This process continues until the end of the episode. 

% \gcx{definition of augmented traj}
% $$
% \tau = \{\ldots, \hat{R}_t, s_t, a_t, \hat{R}_{t+1}, s_{t+1}, a_{t+1}, \ldots\}.
% $$
% The trajectories are augmented with return-to-go tokens $\hat{R}_t$, a quantity that sums up the reward along the future part of the trajectory, which indicates the quality of the action in the immediate steps. During testing, DT specifies a desired target return as the initial RTG $\hat{R}_0$, and acts by auto-regressively predicting the next action given the past states and RTGs. 

==> text/3.defects.tex <==
Existing DT algorithms are commonly implemented by RTG conditioning. Although RTG conditioning is relatively simple to implement, this naive choice has several defects. 

\textbf{Dependency on future trajectory. }
The calculation of RTG involves summing up the rewards in the future trajectory. However, in real-world scenarios, the sampling process is often susceptible to unexpected events, making it challenging to gather complete and continuous trajectories. Under such circumstances, the collected offline dataset may consist of broken snippets of trajectories or even independent transition tuples $(s,a,r,s')$, making it difficult to calculate RTG since the future is missing. As illustrated in Figure~\ref{fig:dt_chunk}, if we divide the trajectories into chunks, DT's performance will degenerate severely. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/dt-chunk.pdf}
    \caption{The performance of DT when the trajectory is divided into chunks. \textit{Chunk\_size} denotes the granularity of division, and \textit{full} means the complete trajectory is preserved. }
    \label{fig:dt_chunk}
\end{figure}



% has two types of limitations. First of all, in real-world scenarios, the sampling process of the behavioral policy is often susceptible to the influence of unexpected events, making it challenging to gather complete and continuous trajectories. Under such circumstances, the collected offline dataset may consist of broken snippets of trajectories or even independent transitions, making it difficult to label RTG since the future is missing. Secondly, during testing, there is also a risk of choosing an inappropriate RTG since we hope to improve beyond the dataset. In Figure~\ref{sec3:fig_dt_defect1} we plot the test performance~(blue line) of DT conditioning on various $\hat{R}_0$~(x-axis) as well as the histogram of the returns of the offline dataset. As we can see, there is no clear pattern for choosing the optimal RTG, for example, although giving a slightly over-estimated RTG hurt the performance in the hopper medium dataset, it actually improves in the walker2d medium-replay dataset. 

% \begin{figure}[htbp]    
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/dt-defect1.pdf}
%     \caption{Illustration on the correlation between RTG, test performance, and dataset histogram for Decision Transformer. }
%     \label{sec3:fig_dt_defect1}
% \end{figure}


\textbf{Inability to perform stitching. }
A well-established consensus on why offline RL methods outperform imitation learning is that they can perform \textit{trajectory stitching}~\cite{why_offlinerl_is_better}, i.e. concatenating multiple snippets of trajectories together to give better performance. However, as pointed out in recent works~\cite{qdt,edt}, DT lacks stitching ability, because the RTG is only associated with the current trajectory. Although conditioning on high RTGs might skew the generated action towards better ones, the performance of DT still falls behind traditional offline RL methods. 

\textbf{Failure in stochastic environments. }
The last failure mode of DT relates to its propensity to make optimistic decisions in stochastic settings, which arises from the intrinsic feature of RTG conditioning to imitate previous achievements indiscriminately while disregarding the randomness.

This phenomenon is also termed the conflation of the effects of the policy and the world model~\cite{doc}, meaning that RTG fails to distinguish the controllable parts (the policy) from the uncontrollable parts (the dynamics) and, as a result, biases the action generation with blind optimism.


==> text/4.method.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/arch.pdf}
    \caption{The architecture of ACT. Different from DT, ACT adopts an encoder-decoder architecture. The encoder encodes the historical state-action sequence into a continuous representation. The attentive head of the decoder queries historical representation with the advantage and predicts an action.}
    \label{fig:arch}
\end{figure*}

\section{Advantage-Conditioned Transformer}

The previous discussion motivates us to devise a better alternative in place of RTG. Observing that dynamic programming handles these challenges effectively, we decide to exploit it for conditional generation. 

Specifically, we approximate the value function via approximate dynamic programming~(Section~\ref{sec4.1}) and estimate advantages with the learned value functions.
After labeling the dataset with advantages~(Section~\ref{sec4.2}), we fit an encoder-decoder transformer on the advantage-augmented dataset via the action reconstruction loss~(Section~\ref{sec4.3}).
We additionally train a predictor $c_\phi$ to estimate the maximal advantage in samples and condition the action generation on the estimated maximum advantage during testing.
The complete algorithm is presented in Algorithm~\ref{algorithm}.

\subsection{Value Function Approximation}\label{sec4.1}
% RTG $\hat{R}=\sum_{t'=t}^{T}r_{t'}$ can be interpreted as an one-sample estimate of the expected return at the given state, it is affected by the stochasticity of both the policy and the environment. Instead, we switch to estimating the value via temporal difference and dynamic programming. 

We use two parameterized functions $Q_\theta$ and $V_\psi$ to approximate the state-action value function and the state value function, respectively. With the offline dataset, we iteratively update the parameters via stochastic gradient descent,
\begin{equation}\label{eq:dp}
\small{
\begin{aligned}
    &\theta\gets \theta-\frac{\eta}{M}\sum_{(s,a,r,s')\in\mathcal{B}}\nabla_\theta\left(Q_\theta(s, a)-r - \gamma V_{\psi_k}(s')\right)^2,\\
    &\psi\gets \psi-\frac{\eta}{M}\sum_{(s,a,r,s')\in \mathcal{B}}\nabla_\psi\mathcal{L}_{\sigma_1}\left(r+\gamma V_{\psi_k}(s') - V_\psi(s)\right), 
\end{aligned}
}
\end{equation}
% \begin{equation}\label{eq:dp}
%     \begin{aligned}
%     \hat{Q}^{k+1}&\leftarrow \arg\min_{Q}\mathbb{E}_{(s, a, s', r)\sim\mathcal{D}}\left[\frac 12 \left(r + \gamma \hat{V}^k(s') - Q(s, a)^2\right)\right]\\
%     \hat{V}^{k+1}&\leftarrow \arg\min_{V}\mathbb{E}_{(s, a, s', r)\sim \mathcal{D}}\left[\mathcal{L}_{\sigma_1}\left(r+\gamma \hat{V}^k(s') - V(s)\right)\right], 
%     \end{aligned}
% \end{equation}
where $\mathcal{B}=\{(s_i,a_i,r_i,s'_i)\}_{i=1}^M$ denotes a mini-batch of transition tuples sampled uniformly from the dataset $\mathcal{D}$, $M$ is the batch size, $\eta$ is the learning rate, $\sigma_1$ is a hyper-parameter, and $\mathcal{L}_{\sigma_1}(u) = |\sigma_1 - \mathbb{I}(u<0)|u^2$ is the expectile regression loss.

% that $(s,a,r)$ are distributed according to the empirical distribution
% $$
% \frac{1}{\sum_{k=1}^MN_k}\sum_{k=1}^M\sum_{i=1}^{N_k}\delta_{(s_t,a_t,r_t)}
% $$
% with the consecutive state $s'$ appended to the end, where $\delta_x$ is delta function centered at $x$ with $\delta_x(x')=\mathbb{I}(x=x')$.

Equation~\eqref{eq:dp} performs in-sample value iteration as outlined by~\citet{iql} which does not query out-of-distribution actions as classical value iteration does. When $\sigma_1$ equals $0.5$, it is conducting on-policy value evaluation, producing an approximation of $Q^\beta$ and $V^\beta$. With infinite samples and $\sigma_1 \to 1$, it produces an approximation of the in-sample optimal value functions: 
$$
    \begin{aligned}
    V_\beta^*(s)&=\max\nolimits_{\beta(a|s)>0} Q_\beta^*(s,a),\\
    Q_\beta^*(s, a)&=\mathcal{R}(s,a)+\gamma\mathbb{E}_{s'\sim T(\cdot|s,a)}\left[V_\beta^*(s')\right].
    \end{aligned}
$$
Thus, this learning procedure smoothly interpolates between approximating on-policy value functions and the in-sample optimal value functions by varying the value of $\sigma_1$. 

Upon the convergence of the training, we freeze $\theta$ and $\psi$ and do not make further updates to them. 

\subsection{Advantage Labeling}\label{sec4.2}
In the next step, we utilize the pre-trained value function approximation to tag the offline data with their advantage. The most straightforward advantage estimator $\hat{A}_{\text{IAE}}$ is simply the difference between $Q_\theta$ and $V_\psi$:
$$
    \begin{aligned}
    \hat{A}^{\text{IAE}}_t = Q_\theta(s_t, a_t) - V_\psi(s_t). 
    \end{aligned}
$$
We term this \textit{Immediate Advantage Estimation}~(IAE). Since $Q_\theta$ averages all subsequent random variations, IAE produces an estimator robust to stochasticity.

However, IAE issues a demand on estimating the state-action value function, which, compared to the state value function, has higher dimensional input and is more difficult to estimate.
Besides, solely depending on Temporal Difference~(TD) error to optimize the value functions is known to fail in sparse-reward or goal-oriented tasks~\cite{qdt, dwsl}.
Thus, we propose to use the \textit{Generalized Advantage Estimation}~(GAE)~\cite{gae} as an alternative:
$$
    \hat{A}^{\text{GAE}(\lambda)}_t =(1-\lambda)\sum_{l=1}^\infty \lambda^{l-1}\hat{A}^{(l)}_t,
$$
where $\hat{A}^{(l)}_t=-V_\psi(s_t)+\sum_{i=0}^{l-1} \gamma^{i}r_{t+i}+\gamma^lV_\psi(s_{t+i+1})$ denotes the $l$-step advantage along the given trajectory. Note that GAE can be extended to the finite horizon case, though we present the infinite horizon formulation here for simplicity. The hyper-parameter $\lambda\in[0,1]$ interpolates between TD estimation and Monte-Carlo estimation, controlling the bias-variance trade-off. With $\lambda$ set to $1$, we have $\hat{A}^{\mathrm{GAE}(1)}_t=\sum_{i=0}^\infty\gamma^i r_{t+i} - V_\psi(s_t)$, which is functionally equivalent to the discounted RTG, since the constant $-V_\psi(s_t)$ does not count when comparing actions.

After deciding on the form of advantage estimator, we label the offline dataset with their advantages, and construct the advantage-augmented dataset $\mathcal{D}^{\mathrm{A}}=\{\tau_k^{\mathrm{A}}\}_{k=1}^{M}$, where $\tau^{\mathrm{A}}_k = \{\hat{A}_t^k, s_t^k, a_t^k\}_{t=0}^{N_k-1}$, and $\hat{A}_t^k$ is the estimated advantage at the $t$-th timestep of the $k$-th trajectory by either IAE or GAE.

\subsection{Advantage-Conditioned Sequence Modeling}\label{sec4.3}
The original DT straightforwardly applies the GPT-2 architecture to RL sequence modeling, offering convenience but falling short of optimization for decision-making tasks.
In our experiments, we observed that modeling using GPT-2 architecture causes overfitting and unstable generation during testing, aligning well with recent research findings~\cite{unimask}.
In light of this, we propose an encoder-decoder transformer architecture illustrated in Figure~\ref{fig:arch}.


In our architecture, the encoder only accepts the state-action sequence as input and applies a causal attention mechanism~\cite{attention_is_all_you_need} to mask out future inputs. It transforms the input sequence $(s_{<t}, a_{<t}, s_t)$ to a representation sequence, where $s_{<t}$ and $a_{<t}$ denote the states and actions before timestep $t$, respectively. 
With cross attention, the decoder queries historical representation with the estimated advantage $\hat A_t$ of the current timestep and predicts an action $\hat a_t$.
The complete function is represented as $\hat{a}_t=\texttt{ACT}(s_{<t}, a_{<t}, s_t, \hat{A}_t)$. 
We found that the separation of the state-action sequence and the advantage benefits the overall performance. Moreover, such separation leaves room for self-supervised pre-training. We may pre-train the encoder using a large unlabelled dataset by techniques similar to Masked Language Modeling~(MLM), reinitialize the decoder, and fine-tune the transformer to accomplish control tasks~\cite{smart, unimask}. 

Another change we made is using the sinusoidal positional encoding in place of learnable positional embedding because we found the latter one sometimes causes overfitting, which echoes the finding by~\citet{onlinedt}. Other details are deferred to Appendix~\ref{app:arch_and_params_act} due to the limitation of space. 

The loss for training ACT is the action reconstruction loss,
\begin{equation}\label{eq:act_objective}
    \mathcal{L}_{\mathrm{ACT}}=\mathbb{E}_{\tau^{\mathrm{A}}\sim\mathcal{D}^{\mathrm{A}}}\left[\sum_{t}(a_t-\texttt{ACT}_\xi(s_{<t}, a_{<t}, s_t, \hat{A}_t))^2\right],
\end{equation}
where $\tau^{\mathrm{A}}\sim\mathcal{D}^{\mathrm{A}}$ means sampling $\tau^{\mathrm{A}}$ uniformly from $\mathcal{D}^{\mathrm{A}}$. 

Finally, similar to DT, we need to specify the target advantage for each state during testing. We additionally train a predictor network $c_\phi$ with the expectile regression loss,
\begin{equation}\label{eq:condition_objective}
    \begin{aligned}
    \mathcal{L}_{\phi}=\mathbb{E}_{(\hat{A}_t, s_t)\sim \mathcal{D}^{\mathrm{A}}}\left[\mathcal{L}_{\sigma_2}\left(\hat{A}_t - c_\phi(s_t)\right)\right],
    \end{aligned}
\end{equation}
where $(\hat{A}_t, s_t)\sim \mathcal{D}^{\mathrm{A}}$ denotes that $(\hat{A}_t, s_t)$ is sampled uniformly from $\mathcal{D}^{\mathrm{A}}$. In the limit of $\sigma_2\to1$, $c_\phi$ learns to predict the maximal in-sample advantage $\max_{\beta(a|s)>0}A^{\pi_{\mathrm{old}}}(s,a)$ given state $s$, which fully exploits ACT's potential in generating a good action. 

\subsection{Why Advantage Conditioning Offers Benefits?}\label{sec4.4:benefits}
In this section, we provide an explanation to why advantage conditioning offers benefits over RTG conditioning.

Recall that, according to the Performance Difference Lemma \cite{policy_difference_lemma},  the performance difference between two policies $\pi$ and $\pi'$ can be expressed as the expected advantage w.r.t. $\pi'$ on the state-action distribution induced by $\pi$, $\eta(\pi)-\eta(\pi')=\mathbb{E}_{\tau\sim\pi}\left[\sum_{t=0}^{\infty}\gamma^t A^{\pi'}(s_t, a_t)\right]$. Assume that our learners are exempt from estimation and approximation errors. If we train ACT with the advantage of the policy $\pi'$ so that, conditioned on a desired advantage $A$, ACT could generate an action $a$ satisfying $A^{\pi'}(s,a)=A$, then we can construct a policy $\pi$ improved over $\pi'$ by providing ACT with a positive target advantage. The expected improvement of $\pi$ over $\pi'$ is specified by the performance difference lemma.
As discussed previously, with $\sigma_1=0.5$, the learned value function approximates the value function of the behavior policy $\beta$, i.e., $\pi'=\beta$. If $\sigma > 0.5$, then the estimated advantage corresponds to a policy $\pi'$ that are already improved over $\beta$.

Since RTGs are Monte-Carlo value estimates for the value of the behavior policy $\beta$, DT is restricted to improve on top of $\beta$, which limits the potential for improvement compared with ACT. Moreover, RTGs suffer from high variance, often assigning high values to actions due to occasional factors, while advantage offers a more robust action assessment by taking the expectation of the future. 


% Older version

% \subsection{Test-time Decoding}
% After fitting on the labeled dataset, ACT is capable of generating a corresponding action given a target advantage and the past trajectory. According to policy difference lemma~\cite{policy_difference_lemma}, the expected improvement of policy $\pi_{\mathrm{new}}$ over policy $\pi_{\mathrm{old}}$ is calculated by
% $$
%     \begin{aligned}
%     J(\pi_{\mathrm{new}}) - J(\pi_{\mathrm{old}})= \mathbb{E}_{\pi_{\mathrm{new}}}\left[\sum_{t=1}^\infty\gamma^{t-1}A^{\pi_{\mathrm{old}}}(s_t, a_t)\right].
%     \end{aligned}
% $$

% Supposing that ACT is supplied with a positive target advantage, and it makes accurate predictions, then an improvement over the old policy $\pi_{\mathrm{old}}$ is guaranteed. Here, the old policy is the policy corresponding to the advantage. As discussed previously, it corresponds to the behavior policy $\beta$ if $\sigma_1=0.5$ and to the in-sample optimal policy in the limit of infinite samples and $\sigma_1\to1$.

% Simply feeding a pre-determined positive target advantage cannot fully unleash the potential of ACT. Therefore we employ another network $c_\phi$ to approximate the maximal in-sample advantage through expectile regression. The function $c_\phi$ is learned by

% where pair of $(\hat A_t,s_t)$ is sampled from the dataset uniformly. 
% % $$
% % \frac{1}{\sum_{k=1}^MN_k}\sum_{k=1}^M\sum_{i=1}^{N_k}\delta_{(\hat A_t, s_t)}
% % $$
% % defined by the dataset $\mathcal{D}^{\mathrm{A}}$.

% In the limit of $\sigma_2\to1$, $c_\phi$ learns to predict the maximal in-sample advantage $\max_{\beta(a|s)>0}A^{\pi_{\mathrm{old}}}(s,a)$ given state $s$.
% We further discuss the test-time decoding and policy improvement in Appendix~\ref{app:test-time_policy_improvement}.


\begin{algorithm}[t]
\caption{Advantage-Conditioned Transformer}
\label{algorithm}
\textbf{Input}: Initialized value networks $Q_\theta, V_\psi$, predictor network $c_\phi$, transformer \texttt{ACT}, offline dataset $\mathcal{D}$ 
\begin{algorithmic}[1]
\STATE // Training Phase
\FOR{$k=1, 2, \ldots, K$}
\STATE Update $Q_\theta$ and $V_\psi$ by Equation~\eqref{eq:dp} on dataset $\mathcal{D}$
\ENDFOR
\STATE Label the dataset $\mathcal{D}$ with estimated advantages to get the advantage-augmented dataset $\mathcal{D}^{\mathrm{A}}$
\STATE Learn \texttt{ACT} by minimizing Equation~\eqref{eq:act_objective} via stochastic gradient descent on dataset $\mathcal{D}^{\mathrm{A}}$
\STATE Learn $c_\phi$ by minimizing Equation~\eqref{eq:condition_objective} via stochastic gradient descent on dataset $\mathcal{D}^{\mathrm{A}}$
\STATE
\STATE // Test Phase
\STATE Initialize history $h=\emptyset$
\WHILE{episode not ended at timestep $t$}
    \STATE Let $A_t=c_\phi(s_t)$
    \STATE Execute $a_t=\texttt{ACT}(h, s_t, A_t)$
    \STATE Update $h=h\cup\{s_t, a_t\}$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> text/5.evaluations.tex <==


\section{Experimental Evaluations}\label{sec6}
Our assessments are designed to comprehensively analyze the efficacy of ACT when presented with diverse benchmarks and tasks encompassing a spectrum of characteristics and challenges. We compare ACT against baseline methods on deterministic, stochastic, and delayed reward tasks. We also conduct an ablation study on the use of network $c_\phi$ and the choice of transformer architecture.

\textbf{Deterministic Gym MuJoCo tasks. }We investigate the performance of ACT in the most widely studied Gym MuJoCo tasks. We focus on three domains, namely \textit{halfcheetah}, \textit{hopper}, and \textit{walker2d}, which are deterministic both in state transition and reward functions. We leverage the \textit{v2} datasets provided by D4RL~\cite{d4rl}, which includes three levels of quality: \textit{medium}, \textit{medium-replay}, and \textit{medium-expert}. 

For this benchmark, we choose GAE(0) as the advantage estimator across all tasks to maximize the utility of dynamic programming. For $\sigma_1$, we sweep its value through $[0.5, 0.7]$. In order to mitigate the instability of TD learning~\cite{regulation}, we conduct model selection by choosing a value model that has the lowest training error on offline dataset. See Appendix~\ref{app:impl_deterministic} for details. 

We contrast the performance of ACT against two groups of algorithms. The first group, including CQL~\cite{cql}, IQL~\cite{iql}, Onestep-RL~\cite{onestep_rl}, 10\%-BC, and RvS~\cite{rvs}, optimizes a Markovian policy that depends only on states. The second group, including DT~\cite{dt}, QDT~\cite{qdt}, and EDT~\cite{edt}, models the RL trajectories with sequence-modeling methods and learns a non-Markovian policy that depends on history. 


% is conditional BC, including 10\%-BC and RvS~\cite{rvs}. The second group is previous RL methods, including CQL~\cite{cql}, IQL~\cite{iql} and Onestep-RL~\cite{onestep_rl}. Finally, the third group is sequence-modeling methods, including Decision Transformer~\cite{dt}, QDT~\cite{qdt}, EDT~\cite{edt} and RvS~\cite{rvs}. 
 
% We contrast the performance of ACT against DP-based methods, including CQL~\cite{cql}, IQL~\cite{iql}, Onestep-RL~\cite{onestep_rl}, and BC-based methods including 10\%-BC, Decision Transformer~\cite{dt}, QDT~\cite{qdt}, EDT~\cite{edt} and RvS~\cite{rvs}. 

The results are listed in Table~\ref{tab:deterministic_gym_perf}. We find that ACT achieves the highest score in 8 out of 9 tasks compared to other methods that learn non-Markovian policies, including QDT and EDT which share a similar motivation with us, i.e., improving DT with the ability of trajectory stitching. The improvement over these methods underscores the efficacy of advantage conditioning. If we extend the comparison to all methods, ACT still manages to outperform in 6 out of 9 tasks. This demonstrates that ACT not only exploits the power of DP but also gains benefits from the sequence modeling technique, thus combining the best of both worlds. 

% \begin{figure*}[htbp]
%     \centering
%     \subfigure[2048 Game]{
%     \includegraphics[width=0.44\linewidth]{figures/2048_perf.pdf}
%     }
%     \subfigure[Stochastic Gym MuJoCo]{
%     \includegraphics[width=0.51\linewidth]{figures/stoc_mujoco_perf.pdf}
%     }
%     \caption{Performance on stochastic benchmarks, including the 2048 game~(discrete control) and the customized stochastic MuJoCo tasks~(continuous control). The solid line represents the average performance while the shaded area represents one standard deviation of the performance across five seeds. }
%     \label{fig:stochastic_perf}
% \end{figure*}
\input{tables/deterministic_mujoco_perf.tex}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/2048_perf.pdf}
    \caption{Performance on the 2048 game. We report the average and std of the performance across 5 independent runs and mark ESPER's score as the grey dotted line. }
    \label{fig:2048_perf}
\end{figure}

\textbf{Stochastic benchmarks. }Another important property of ACT is its robustness against the stochasticity of the environments. To validate this, we choose to assess ACT, DT, ESPER~\cite{esper}, and 10\%-BC on stochastic benchmarks. Among them, ESPER is an algorithm that enhances DT to cope with environmental stochasticity. In the following evaluations, we select IAE as the advantage estimator, and $\sigma_1$ is kept to 0.5 by default. 



As a sanity check, we first evaluate the algorithms on the 2048 game. This environment is stochastic in that, after each action which moves all the tiles along some direction and merges them if their numbers are equal, a random 2 or 4 will be placed in a random empty grid. The agent is given a reward of 1 once it manages to produce a tile of 128, and the episode will be ended. Thus, the maximum return in this environment is 1. Further introduction about this environment and the dataset can be found in Appendix~\ref{app:impl_2048}. 
% The offline dataset consists of a total number or 5M steps collected by a random policy and an expert policy. 
Figure~\ref{fig:2048_perf} depicts the performance curve as the training proceeds. While DT and 10\%-BC exploit the occasional success in the dataset and converge to suboptimal policies, ACT and ESPER show robustness to stochasticity. Besides, ACT outperforms ESPER and converges to 100\% success rate to produce 128, validating the power of advantage conditioning. 

We also created a more sophisticated benchmark, by reusing the Gym MuJoCo tasks and following \citet{doc} to add noise to the agent's action before passing it to the simulator. More details can be found in Appendix~\ref{app:impl_stochastic}. The results are illustrated in Figure~\ref{fig:stoc_mujoco_perf}. As expected, we observe that 10\%-BC severely overfits the high-return trajectories in the dataset, albeit with a sharp drop in test scores as the training proceeds. DT yields a comparatively robust policy, while its performance is still inferior to ACT. This further justifies the validity of ACT in stochastic control tasks. 



% we created a range of environments with stochastic state transitions similar to~\cite{doc}. To be specific, we reuse the Gym MuJoCo tasks and add independent Gaussian noise to the actions of the agent. The noise is sampled from a zero-meaned Gaussian distribution with the standard deviation being $1-\exp(-0.01t)\cdot 0.35\sin(t)$, where $t$ stands for the timestep. The agent is not aware of the noise and thus from its perspective, the environment becomes stochastic since the outcome of the same action is not fixed. The offline data is collected by a pre-trained expert policy or a medium policy whose performance is approximately 30\% of the expert. More details can be found in Appendix~\ref{app:impl_stochastic}. 

% Considering the stochasticity, we select IAE as the advantage estimator and $\sigma_1$ is kept as $0.5$ by default. We select two behavior cloning methods, namely 10\%-BC and DT as baselines, and the results are illustrated in Figure~\ref{exp:fig_stochastic}. As expected, 10\%-BC severely overfits the trajectories with the top 10\% empirical returns in the dataset, albeit erroneously. Thus, we witness a sharp drop in the test performance of 10\%-BC as the training proceeds. DT yields a more robust policy, while its performance is still inferior compared to ACT. This validates the robustness of ACT when confronted with environmental stochasticity. 

\input{tables/delayed_perf.tex}


\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/stoc_mujoco_perf.pdf}
    \caption{Performance curve the stochastic Gym MuJoCo tasks as the training proceeds. We report the average and the standard deviation of the performance across 4 independent runs. }
    \label{fig:stoc_mujoco_perf}
\end{figure*}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/abl_sigma2_perf_new.pdf}
    \caption{Ablation study on the effect of $\sigma_2$, using datasets from D4RL. The left column depicts the performance of each variant as the training proceeds, and the right column depicts the target advantages given by $c_\phi$. The results are taken from 4 independent runs.}
    \label{fig:abl_sigma2}
\end{figure}

\textbf{Delayed reward tasks. }As unveiled in previous literature~\cite{dt, qdt}, DT has an advantage over conventional RL methods when the reward is sparse and thus long-term credit assignment is required. In the following part, we aim to investigate whether ACT still retains such ability. We once again revise the D4RL datasets, deferring the rewards for each trajectory until the final timestep. We exclude the \textit{halfcheetah} and \textit{medium-replay} datasets as they contain time-out trajectories which are not applicable for delayed-reward settings. For the advantage estimator, we choose GAE(1) for its resemblance to the RTGs. The results are listed in Figure~\ref{tab:delayed_perf}. While DP-based methods such as CQL and IQL suffer from degeneration, DT upholds its performance and is minimally affected by reward sparsity. Although ACT is not entirely spared from the influence, it still preserves benefits from the sequence modeling architecture and outperforms CQL and IQL. 

\textbf{Ablation study. }
Finally, we investigate the effects of the design choices of ACT through ablation studies. Our first ablation focuses on the effect of $\sigma_2$, which determines the expectile that our predictor network $c_\phi$ tries to approximate. In the above experiments, we set the $\sigma_2$ to $0.98$, and in this ablation study, we additionally test the values, $0.5$, $0.7$, and $0.9$ to analyze the actual effect of this parameter. According to the discussions in Section~\ref{sec4.4:benefits}, providing ACT with a positive advantage already induces policy improvement. Therefore we also include a variant of ACT which uses a constant positive value as the target advantage for all states. The positive value is set as the average of the positive advantages in the offline dataset.
The result illustrated in Figure~\ref{fig:abl_sigma2} suggests a close relationship between the value of $\sigma_2$ and the final performance.
When $\sigma_2$ is set to higher values, the predictor network $c_\phi$ tends to give higher desired advantages $\hat{A}$ during test time, and ACT would  retrieve better actions in response. 
Giving a positive constant value also brings about improvement in certain environments such as \textit{halfcheetah-medium}, but in \textit{hopper-medium} it performs substantially worse than using a predictor network. For comparisons on more tasks and datasets, please refer to Appendix~\ref{app:more_perf_abl_sigma2}.  

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/ablation_arch.pdf}
    \caption{Ablation study on the transformer architecture, using datasets from D4RL with 4 independent runs.}
    \label{fig:abl_arch}
\end{figure}

We also carried out an analysis of the choice of transformer architecture. The architecture of ACT differs from DT in two ways: 1) ACT employs an encoder-decoder structure while DT is a decoder-only transformer, and 2) ACT uses sinusoidal encoding rather than learnable embedding to prevent overfitting. Thus, we additionally implement two variants of ACT, one with GPT-2 architecture~(\texttt{ACT-GPT}) and another using learnable positional embedding~(\texttt{ACT-Embed}), and keep other hyper-parameters the same with \textit{ACT}. We contrast their performance in Figure~\ref{fig:abl_arch}. 
We select the \textit{medium-replay} and \textit{medium-expert} datasets of the hopper task for illustration, and the full comparison is deferred to Appendix~\ref{app:more_perf_abl_arch}.
We can observe that \texttt{ACT-GPT} has undergone significant oscillation and degradation in its performance, implying that the direct application of GPT-2 structure to our algorithm is not effective. The other variant, \texttt{ACT-Embed}, suffers from instabilities in tasks like \textit{hopper-medium-expert} in the late training, although the overall gap is minor. 


==> text/6.related_work.tex <==
\textbf{Dealing with stochastic environments for DT. }
Numerous related works are dedicated to addressing the vulnerability of DT when confronted with stochastic environments.
ESPER~\cite{esper} uses adversarial clustering to learn trajectory representations disentangled from environmental stochasticity.
DoC~\cite{doc} identifies the root cause of such failure is that generative models make no distinction between the parts it can control~(agent actions) and those it cannot~(environmental transition).
Thus, DoC proposes to extract predictive representations for trajectories, while minimizing the mutual information between the representation and the environment transition.
A similar idea is also explored in~\cite{optimism_bias}, where the authors explicitly model the policy and the world model with two separate transformers.
\citet{rcsl_dp_analysis} provided a theoretical analysis of the return-conditioning regime, where they found the near-determinism of the environment is one of the conditions that return-conditioning can find the optimal policy. 

\textbf{Combining DP and DT. }Most of the offline RL methods employ dynamic programming to optimize policies, such as CQL~\cite{cql}, IQL~\cite{iql}, and TD3+BC~\cite{td3bc}.
As discussed in this paper as well as in \citet{rcsl_dp_analysis}, DP and DT bear distinct characteristics, for example, DP has no preference for the determinism of the environment, while DT may be more applicable in long-horizon tasks.
Several works have tried to combine DP and DT.
Among them, QDT~\cite{qdt} pre-computes conservative Q-values and V-values using CQL, and labels the offline data with the maximum of RTG and the conservative V-value. Our method differs from QDT in that, we compute the value estimations via an in-sample value iteration, which prevents instability and inaccuracy caused by bootstrapping from out-of-dataset actions. Moreover, the flexible advantage estimation also enables ACT to combine the best of both worlds.
Recently, EDT~\cite{edt} was proposed to vary the context length of DT during testing. When provided a shorter context, EDT can recover from bad history and switch to a higher rewarding action; provided a long context, EDT can stably recall the subsequent decisions.
In this way, EDT interpolates between trajectory stitching and behavior cloning from a new perspective. This work is complementary to ACT, and they can be seamlessly integrated to achieve better performance. 

==> text/7.conclusion.tex <==
In this paper, we introduced Advantage-Conditioned Transformer, which enhances popular sequence modeling techniques with dynamic programming to address their limitations in offline policy optimization. We achieve this by conditioning the transformer architecture on the estimated advantages. 
% Specifically, we leverage dynamic programming to estimate the value functions on offline data. Subsequently, we propose two classes of advantage estimators, namely IAE and GAE, to obtain the advantage for actions within the offline dataset. Finally, we switch from conditioning the transformer structure on RTG to conditioning on the estimated advantages. 
By selectively choosing the type of advantage estimator, our framework can be applied to a variety of tasks, demonstrating consistent performance improvements and generalizability. Our framework also leaves room for the incorporation of self-supervised learning~(SSL) techniques and has the potential to be extended to multi-task settings and to a larger training scale. We will continue this line of research and investigate these topics in the future. 
